Beyond Hard Samples: Robust and Effective Grammatical Error Correction with Cycle Self-Augmenting

Recent studies have revealed that grammatical error correction methods in the sequence-to-sequence paradigm are vulnerable to adversarial attack, and simply utilizing adversarial examples in the pre-training or post-training process can significantly enhance the robustness of GEC models to certain types of attack without suffering too much performance loss on clean data. In this paper, we further conduct a thorough robustness evaluation of cutting-edge GEC methods for four different types of adversarial attacks and propose a simple yet very effective Cycle Self-Augmenting (CSA) method accordingly. By leveraging the augmenting data from the GEC models themselves in the post-training process and introducing regularization data for cycle training, our proposed method can effectively improve the model robustness of well-trained GEC models with only a few more training epochs as an extra cost. More concretely, further training on the regularization data can prevent the GEC models from over-fitting on easy-to-learn samples and thus can improve the generalization capability and robustness towards unseen data (adversarial noise/samples). Meanwhile, the self-augmented data can provide more high-quality pseudo pairs to improve model performance on the original testing data. Experiments on four benchmark datasets and seven strong models indicate that our proposed training method can significantly enhance the robustness of four types of attacks without using purposely built adversarial examples in training. Evaluation results on clean data further confirm that our proposed CSA method significantly improves the performance of four baselines and yields nearly comparable results with other state-of-the-art models. Our code is available at https://github.com/ZetangForward/CSA-GEC.

==> adding.tex <==
\subsection{Data Usage Analysis}
\subsubsection{Training Data for Three Training Stage}

% Observed by \citep{kiyono2019empirical,omelianchuk2020gector}, having two fine-tuning stages with a perspective dataset is crucial for performance. However, there is no theoretical reason for this phenomenon ,and the relationship between $D_{tune}$ and regularization data requires thorough study. In this section, we will first analyze the function of relatively small magnitude and realistic dataset $D_{tune}$ from the perspective of optimization objective and generalization. Then, we will explain the rationality of our strategy by comparing between several candidate strategies.

\subsubsection{Function of $D_{tune}$ for Performance}
As mentioned 


\subsubsection{Regularization Data During the Cycle}



\subsubsection{Comparison between Different Cycle Strategy}

==> relate_work.tex <==

\section{Related Work}
\label{sec:related_work}

\subsection{Layout Generation}
\label{subsec:layout_gen}
Automatic layout generation, an important task for automatic graphical design for various scenarios such as document layouts~\citep{zheng2019content,zhong2019publaynet,yamaguchi2021canvasvae,fu2022doc2ppt}, posters~\citep{yang2016automatic,guo2021vinci,li2023relation} and user interface~\citep{deka2017rico}, has been recently extensively researched. 
Early approaches for layout generation involve embedding design rules into manually-defined energy functions~\citep{o2014learning,o2015designscape}, while other methods have explored generative models such as GANs and VAEs for generating numerical graphic and scene layouts, including LayoutGAN~\citep{li2019layoutgan}, LayoutVAE~\citep{jyothi2019layoutvae}, LayoutGAN++~\citep{kikuchi2021constrained}, NDN~\citep{lee2020neural} and READ~\citep{patil2020read}.
Apart from them, transformer-based approaches utilize self-attention mechanisms to learn numerical contextual relationships between elements and achieve layout completion based on partial layout inputs~\citep{yang2020layouttransformer,kong2022blt,feng2023layoutgpt}. 
Recently, with the prevalence of diffusion models, several works also adopted diffusion models to tackle a broader range of conditional layout generation~\citep{chai2023layoutdm,inoue2023layoutdm,zhang2023layoutdiffusion,hui2023unifying,cheng2023play}.
However, existing methods primarily treat layout generation as a numerical optimization task, focusing on quantitative aspects while overlooking the semantic information of layout, such as the relationship between each layout element. Different from previous works, we convert the layout generation task into the code generation task to directly generate the layout in code language and thus utilize the rich knowledge from LLMs, which can significantly improve the FID by 50\%  in the Magazine dataset in \cref{subsec:results}.


\subsection{Instruction Tuning}
\label{subsec:instruct_tune}
Instruction tuning represents the process of fine-tuning LLMs on the instruction dataset in a supervised fashion, which narrows the gap between the next-word prediction manner of LLMs and the users' objective of having LLMs adhere to human instructions~\citep{zhang2023instruction}.
Early attempts on instruction tuning involve multi-task training with manually-written descriptions about different tasks~\citep{mishra2021cross,wei2021finetuned,sanh2021multitask,xu2022zeroprompt,muennighoff2022crosslingual,iyer2022opt} or automatically generated instructions~\citep{wang2022self,gu2022learning,zhang2023generation,honovich2022unnatural,honovich2022instruction}.
Apart from controlling the LLMs through input instruction, \citet{nye2021show} show that LLM can handle more complex tasks by generating the intermediate steps and \citet{wei2022chain} propose chain-of-thought technique by enriching the instruction with intermediate reasoning step descriptions, which endows LLMs with better performance~\citep{wang2022self,zelikman2022star,wu2023improving,xu2023wizardlm}.
However, the instruction tuning methods mentioned above are primarily intended for text generation tasks and not ideal for layout generation tasks, which involve numerical optimization. Thus, we propose a code instruction tuning method that is specially designed for layout generation task.
Experiments in \cref{subsec:effect_of_tuning_methods} indicate that the performance significantly drops if the code instruction tuning is not adopted.



==> table/case_forget.tex <==
\begin{table}[hbt!]
\caption{The forgetting phenomenon between stage \uppercase\expandafter{\romannumeral2} and stage \uppercase\expandafter{\romannumeral3} }
\label{tab:forgetting} 
\begin{tabular}{c | c | c c c | c c c }
    \toprule
    \multirow{2}{*}{\shortstack{\textbf{Model}}} & \multirow{2}{*}{\shortstack{\textbf{Cycle}}} & \multicolumn{3}{c}{\textbf{Stage \uppercase\expandafter{\romannumeral2}}} & \multicolumn{3}{c}{\textbf{Stage \uppercase\expandafter{\romannumeral3}}} \\
    \cmidrule(r){3-8} 
     & & \textbf{P} & \textbf{R} & \textbf{F\_{0.5}~~} & \textbf{P} & \textbf{R} & \textbf{F\_{0.5}~~} \\
     \midrule
     \multirow{4}{*}{\shortstack{Transformer \\ \cite{kiyono2019empirical}}}  & 1 & 64.9 & 42.7 & 58.8 & 66.5 & 51.1 & 62.7  \\
     & 2 & 62.5 & 45.9 & 58.2 & 67.2 & 49.4 & 62.6 \\
     & 3 & 64.0 & 43.2 & 58.4 & 67.5 & 49.4 & 62.9 \\
     & 4 & 59.8 & 43.5 & 55.7 & 66.9 & 49.6 & 62.6 \\
     \midrule
     \multirow{3}{*}{\shortstack{Transformer + MI \\ \cite{kaneko2020encoder}}}  & 1 & 65.1 & 45.4 & 59.6 & - & - & -  \\
     & 2 & 64.8 & 46.9 & 60.2 & - & - & -  \\
     & 3 & 65.2 & 45.2 & 59.4 & - & - & -  \\
    
    
    \bottomrule
\end{tabular}
\end{table}


==> table/distance.tex <==
\begin{table}[hbt!]
\caption{The influence of editing distance}
\label{tab:dis} 
\begin{tabular}{c | c | c | c c c}
    \toprule
    \multirow{2}{*}{\shortstack{\textbf{Model}}} & \multirow{2}{*}{\shortstack{\textbf{Cycle}}} & \multirow{2}{*}{\shortstack{\textbf{Editing} \\ \textbf{Distance}}} & \multicolumn{3}{c}{\textbf{Conll2014}} \\
    \cmidrule(r){4-6} 
     & & & \textbf{P} & \textbf{R} & \textbf{F\_{0.5}~~} \\
     \midrule 
     \multirow{2}{*}{\shortstack{Transformer \\ \cite{kiyono2019empirical}}}  & 1 & - & 64.9 & 42.7 & 58.8 \\
     & 1 & - & 66.5 & 51.1 & 62.7  \\
     \midrule
     \multirow{2}{*}{\shortstack{Transformer \\ \cite{kiyono2019empirical}}}  & 1 & 12 & 58.6 & 45.5 & 55.4 \\
     & 1 & 12 & 68.9 & 44.2 & 61.9 \\
     \midrule 
     \multirow{2}{*}{\shortstack{Transformer \\ \cite{kiyono2019empirical}}}  & 1 & 20 & 58.4 & 43.7 & 54.8 \\
     & 1 & 20 & 65.1 & 46.3 & 60.2 \\

    \bottomrule
\end{tabular}
\end{table}


==> table/errorType/error_type_CSA.tex <==
\begin{table}[hbt!]
    \centering
    \caption{Recall of each error type for our \textbf{CSA} method.}
    \begin{tabular}{c|c|c|c|c|c|c}
        \toprule
        \textbf{Error type} & \textbf{Train set 1} & \textbf{Train set 2} & \textbf{Train set 3} & \textbf{Train set 4} & \textbf{Train set 5} & \textbf{Average}  \\
        \midrule
         \bf ADJ &45.5 &50.0 &50.0 &43.5 &42.9 &46.4 \\
         \bf ADV &64.0 &56.3 &59.3 &60.0 &60.0 &59.9 \\
         \bf CONJ &58.3 &37.5 &50.0 &15.4 &81.8 &48.6 \\
         \bf CONTR &100 &100 &33.3 &100 &66.7 &80.0 \\
         \bf DET &30.1 &27.0 &25.2 &31.7 &32.1 &29.2 \\
         \bf MORPH &25.8 &31.0 &21.2 &13.5 &17.0 &21.7 \\
         \bf NOUN &52.4 &57.4 &51.4 &48.5 &62.7 &54.5 \\
         \bf NOUN:NUM &28.0 &13.8 &27.6 &19.1 &29.6 &23.6 \\
         \bf NOUN:POSS &20.0 &28.6 &0.0 &25.0 &0.0 &14.7 \\
         \bf ORTH &0.0 &7.1 &27.3 &46.2 &10.0 &18.1 \\
         \bf OTHER &49.6 &56.5 &53.5 &50.4 &56.0 &53.2 \\
         \bf PART &50.0 &28.6 &0.0 &42.9 &40.0 &32.3 \\
         \bf PREP &34.5 &30.3 &30.5 &34.8 &28.6 &31.7 \\
         \bf PRON &46.7 &52.6 &28.6 &53.3 &33.3 &42.9 \\
         \bf PUNCT &47.3 &38.2 &30.9 &32.7 &38.2 &37.5 \\
         \bf SPELL &14.3 &23.1 &50.0 &31.3 &22.2 &28.2 \\
         \bf VERB &56.3 &55.4 &48.9 &50.0 &57.9 &53.7 \\
         \bf VERB:FORM &29.4 &23.3 &17.1 &21.7 &21.6 &22.6 \\
         \bf VERB:SVA &24.2 &22.0 &13.2 &22.0 &20.6 &20.4 \\
         \bf VERB:TENSE &53.1 &44.9 &42.4 &49.3 &43.0 &46.5 \\
         \bf WO &0.0 &36.4 &37.5 &20.0 &26.7 &24.1 \\
        \bottomrule
    \end{tabular}
    
    \label{tab:error_type}
\end{table}


==> table/errorType/error_type_benchmark.tex <==
\begin{table}[hbt!]
    \centering
    \caption{Recall of each error type for benchmark model.}
    \begin{tabular}{c|c|c|c|c|c|c}
        \toprule
        \textbf{Category} & \textbf{Train set 1} & \textbf{Train set 2} & \textbf{Train set 3} & \textbf{Train set 4} & \textbf{Train set 5} & \textbf{Average}  \\
        \midrule
         \bf ADJ &59.1 &45.8 &57.7 &60.9 &42.9 &53.3 \\
         \bf ADV &60.0  &56.3 &74.1 &50 &52.0 &58.5 \\
         \bf CONJ &58.3  &62.5 &41.7 &46.2 &81.8 &58.1 \\
         \bf CONTR &100  &100 &33.3 &100 &66.7 &80.0 \\
         \bf DET &41.6  &33.7 &35.9 &39.7 &44.2 &39.0 \\
         \bf MORPH &29.0  &31.0 &23.1 &32.4 &17.0 &26.5 \\
         \bf NOUN &57.1  &61.1 &61.1 &62.1 &64.4 &61.2 \\
         \bf NOUN:NUM &38.0  &22.5 &29.3 &27.0 &36.6 &30.7 \\
         \bf NOUN:POSS &20.0  &28.6 &14.3 &25.0 &40.0 &25.6 \\
         \bf ORTH &20.0  &21.4 &36.4 &46.2 &20.0 &28.8 \\
         \bf OTHER &58.5  &61.3 &60.6 &56.6 &60.3 &59.5 \\
         \bf PART &57.1  &50.0 &0.0 &42.9 &60.0 &42.0 \\
         \bf PREP &39.3  &41.6 &37.9 &40.2 &40.5 &39.9 \\
         \bf PRON &46.7  &52.6 &38.1 &46.7 &33.3 &43.5 \\
         \bf PUNCT &54.1  &58.2 &61.8 &63.8 &67.1 &61.0 \\
         \bf SPELL &28.6  &38.5 &50.0 &43.8 &22.2 &36.6 \\
         \bf VERB &57.8  &66.1 &46.8 &44.6 &57.9 &54.6 \\
         \bf VERB:FORM &33.3  &41.9 &19.5 &26.1 &18.9 &27.9 \\
         \bf VERB:SVA &18.2  &24.4 &18.4 &24.4 &20.6 &21.2 \\
         \bf VERB:TENSE &55.6  &43.9 &50.0 &52.0 &48.8 &50.1 \\
         \bf WO &14.3  &45.5 &50.0 &40.0 &53.3 &40.6 \\
        \bottomrule
         
    \end{tabular}
    
    \label{tab:error_type}
\end{table}


==> table/errorType/error_type_train_without_sampling.tex <==
\begin{table}[hbt!]
    \centering
    \caption{Recall of each error type for our \textbf{CSA} method and filter the unlearned data.}
    \begin{tabular}{c|c|c|c|c|c|c}
        \toprule
        \textbf{Error type} & \textbf{Train set 1} & \textbf{Train set 2} & \textbf{Train set 3} & \textbf{Train set 4} & \textbf{Train set 5} & \textbf{Average}  \\
        \midrule
         \bf ADJ &45.5 &45.8 &53.9 &56.5 &42.9 &48.9 \\
         \bf ADV &72.0 &56.3 &70.4 &55.0 &60.0 &62.7 \\
         \bf CONJ &58.3 &25.0 &50.0 &23.1 &72.7 &45.8 \\
         \bf CONTR &100 &66.7 &33.3 &100 &66.7 &73.3 \\
         \bf DET &33.5 &27.5 &26.4 &32.2 &33.2 &30.6 \\
         \bf MORPH &19.4 &28.6 &25.0 &21.6 &19.2 &22.8 \\
         \bf NOUN &58.7 &55.6 &48.6 &59.1 &62.7 &56.9 \\
         \bf NOUN:NUM &31.0 &20.0 &32.8 &23.6 &32.4 &28.0 \\
         \bf NOUN:POSS &20.0 &28.6 &14.3 &25.0 &20.0 &21.6 \\
         \bf ORTH &0.0 &7.14 &18.2 &61.5 &0.0 &17.4 \\
         \bf OTHER &56.6 &53.0 &54.8 &51.5 &55.6 &54.3 \\
         \bf PART &50.0 &35.7 &16.7 &42.9 &50.0 &39.1 \\
         \bf PREP &38.1 &32.6 &29.5 &33.7 &32.1 &33.2 \\
         \bf PRON &46.7 &47.4 &42.9 &46.7 &33.3 &43.4 \\
         \bf PUNCT &48.7 &32.7 &29.1 &34.5 &48.7 &38.7 \\
         \bf SPELL &28.6 &30.8 &50.0 &37.5 &44.4 &38.3 \\
         \bf VERB &51.6 &64.3 &53.2 &46.4 &56.1 &54.3 \\
         \bf VERB:FORM &31.4 &27.9 &22.0 &21.7 &24.3 &25.5 \\
         \bf VERB:SVA &24.2 &24.4 &15.8 &24.4 &17.7 &21.3 \\
         \bf VERB:TENSE &54.3 &40.8 &48.5 &50.7 &43.0 &47.5 \\
         \bf WO &14.3 &36.4 &50.0 &20.0 &40.0 &32.1 \\
        \bottomrule
    \end{tabular}
    
    \label{tab:error_type}
\end{table}


==> table/model_config.tex <==
\begin{table}[hbt!]
\caption{The influence of editing distance}
\label{tab:dis} 
\begin{tabular}{c | c | c | c | c}
    \toprule
    \textbf{Model} & \textbf{Parameters} &  \textbf{GPU} & \textbf{DataSet} & \textbf{BSZ} \\
    \midrule
    Transformer \cite{kiyono2019empirical} & 201,785,344 & A100 $\times$ 8 & Pseudo & 9012^{$\dagger$} \\
    \midrule
    Bert-fuse \cite{kaneko2020encoder} & 354,184,960 & A100 $\times$ 8 & Pseudo & 9012^{$\dagger$} \\
    \midrule
    BART \cite{katsumata2020stronger} & 406,290,432 & A100 $\times$ 8 & Pseudo & 4096^{$\dagger$} \\
    \midrule
    RoBERTa \cite{omelianchuk2020gector} & 124,645,632 & A100 $\times$ 1 & PIE & 512^{$\ddagger$} $\times$ 4 \\
    \midrule
    BERT \cite{omelianchuk2020gector} & 109,482,240 & A100 $\times$ 1 & PIE & 512^{$\ddagger$} $\times$ 4 \\
    \midrule
    XLNet \cite{omelianchuk2020gector} & 116,718,336 & A100 $\times$ 1 & PIE & 512^{$\ddagger$} $\times$ 4 \\
    \bottomrule
\end{tabular}
\end{table}


==> table/pretrain.tex <==
\begin{table}[hbt!]
\caption{The forgetting phenomenon between stage \uppercase\expandafter{\romannumeral2} and stage \uppercase\expandafter{\romannumeral3} }
\label{tab:forgetting} 
\begin{tabular}{c | c | c c c | c c c }
    \toprule
    \multirow{2}{*}{\shortstack{\textbf{Model}}} & \multirow{2}{*}{\shortstack{\textbf{Cycle}}} & \multicolumn{3}{c}{\textbf{Stage \uppercase\expandafter{\romannumeral2}}} & \multicolumn{3}{c}{\textbf{Stage \uppercase\expandafter{\romannumeral3}}} \\
    \cmidrule(r){3-8} 
     & & \textbf{P} & \textbf{R} & \textbf{F\_{0.5}~~} & \textbf{P} & \textbf{R} & \textbf{F\_{0.5}~~} \\
    \midrule
    \multirow{4}{*}{\shortstack{Transformer \\ \cite{kiyono2019empirical}}}  & 1 & 64.9 & 42.7 & 58.8 & 66.5 & 51.1 & 62.7  \\
     & 2 & 62.5 & 45.9 & 58.2 & 67.2 & 49.4 & 62.6 \\
     & 3 & 64.0 & 43.2 & 58.4 & 67.5 & 49.4 & 62.9 \\
     & 4 & 59.8 & 43.5 & 55.7 & 66.9 & 49.6 & 62.6 \\
    \multirow{2}{*}{\shortstack{BERT-fuse \\ \cite{kaneko2020encoder}}}  & 1 & & & & & & \\
    & 2 & & & & & & \\
     
     
    
    
    \bottomrule
\end{tabular}
\end{table}

